Metadata-guided Feature Disentanglement for Functional Genomics

With the development of high-throughput technologies, genomics datasets rapidly grow in size, including functional genomics data. This has allowed the training of large Deep Learning (DL) models to predict epigenetic readouts, such as protein binding or histone modifications, from genome sequences. However, large dataset sizes come at a price of data consistency, often aggregating results from a large number of studies, conducted under varying experimental conditions. While data from large-scale consortia are useful as they allow studying the effects of different biological conditions, they can also contain unwanted biases from confounding experimental factors. Here, we introduce Metadata-guided Feature Disentanglement (MFD) - an approach that allows disentangling biologically relevant features from potential technical biases. MFD incorporates target metadata into model training, by conditioning weights of the model output layer on different experimental factors. It then separates the factors into disjoint groups and enforces independence of the corresponding feature subspaces with an adversarially learned penalty. We show that the metadata-driven disentanglement approach allows for better model introspection, by connecting latent features to experimental factors, without compromising, or even improving performance in downstream tasks, such as enhancer prediction, or genetic variant discovery. The code for our implemementation is available at https://github.com/HealthML/MFD

==> sections/methods/training.tex <==
% \subsection{Model Training}
% We train \ac{MethodName} models on sequences from the GRCh38 human reference genome to predict peak-calls in $\numExperimentsNumeric$ tissue-specific DNA-accessibility (ATAC-seq, DNase-seq) and chromatin modification (ChIP-seq) experiments on human samples from the \ac{ENCODE} database.
% We also obtained metadata and quality metrics for every experiment. We defined sample's tissue, organ, life stage, age, and target (e.g., accessible DNA or chromatin modifications) as biological features and year, laboratory, and assay together with quality metrics as technical metadata features. Details on model training can be found in Appendix~\ref{app:training}, and on data collection and set-up in Appendix~\ref{app:encode_get_data}.

